LACS: Learning-Augmented Algorithms for Carbon-Aware Resource Scaling with Uncertain Demand

Motivated by an imperative to reduce the carbon emissions of cloud data centers, this paper studies the online carbon-aware resource scaling problem with unknown job lengths (OCSU) and applies it to carbon-aware resource scaling for executing computing workloads. The task is to dynamically scale resources (e.g., the number of servers) assigned to a job of unknown length such that it is completed before a deadline, with the objective of reducing the carbon emissions of executing the workload. The total carbon emissions of executing a job originate from the emissions of running the job and excess carbon emitted while switching between different scales (e.g., due to checkpoint and resume). Prior work on carbon-aware resource scaling has assumed accurate job length information, while other approaches have ignored switching losses and require carbon intensity forecasts. These assumptions prohibit the practical deployment of prior work for online carbon-aware execution of scalable computing workload. We propose LACS, a theoretically robust learning-augmented algorithm that solves OCSU. To achieve improved practical average-case performance, LACS integrates machine-learned predictions of job length. To achieve solid theoretical performance, LACS extends the recent theoretical advances on online conversion with switching costs to handle a scenario where the job length is unknown. Our experimental evaluations demonstrate that, on average, the carbon footprint of LACS lies within 1.2% of the online baseline that assumes perfect job length information and within 16% of the offline baseline that, in addition to the job length, also requires accurate carbon intensity forecasts. Furthermore, LACS achieves a 32% reduction in carbon footprint compared to the deadline-aware carbon-agnostic execution of the job.

==> Z-exp-old.tex <==
\begin{table*}[t]
    \centering
    % \scriptsize
    \footnotesize
    \captionof{table}{Summary of evaluated algorithms in the experiments}
    \vspace{-0.3cm}
    \label{table:baseline-algs}
    \begin{tabular}{|c|c|c|c|c|}
    \hline
    \textbf{Algorithm} & \textbf{Carbon-Aware} & \textbf{Switching-Aware} & \textbf{Job Length Input} & \textbf{Compulsory Trading Start Time} \\ \hline
    \RORO \cite{Lechowicz:24} & Yes & Yes & Actual & $T - \frac{(c - w^t)}{r}$  \\ \hline
    \OWT & Yes & No & Prediction & $T - \frac{(\cmax - w^t)}{r}$  \\ \hline
    \threshold & Yes & No & N/A & $T - \frac{(\cmax - w^t)}{r}$  \\ \hline
    \agnostic & No & No & N/A & $T - \frac{(\cmax - w^t)}{r}$  \\ \hline
    \carbonscaler\cite{Hanafy:23:CarbonScaler} & Yes & No & Prediction & $T - \frac{(\cmax - w^t)}{r}$  \\ \hline
    \aug (this paper) & Yes & Yes & Prediction & $T - \frac{(\cmax - w^t)}{r}$  \\ \hline
    \end{tabular}
    \vspace{0.1cm}
\end{table*}

This section evaluates the proposed learning-augmented algorithm \aug in carbon-aware horizontal resource scaling when dealing with uncertain demand, specifically unknown job length. First, we will explain our experimental setup. Then, we will show through numerical analysis how our proposed algorithm outperforms current state-of-the-art methods. Finally, we will evaluate our proposed method under real-world constraints and scenarios. \wa{we no longer have difference between the two parts} 
\subsection{Experimental Setup}
In this work, we follow a job-centric regime to minimize the total $CO_2$ emissions as in ~\cite{Hanafy:23:CarbonScaler}, where the scheduler allocates cloud resources for each job independently while respecting deadlines.

\noindent \textbf{Carbon Trace:}
We use carbon intensity data for California ISO (CAISO) from Electricity Maps~\cite{electricity-map} covering the years 2020 to 2033. Electricity maps provide information on the average carbon emissions in grams of CO2 equivalent per kilowatt-hour (gCO2eq/kWh) at an hourly granularity. \wa{Jobs arrive every 20} We uniformly sample 1300 start times for each experiment to assess the performance across different start times. 
To evaluate algorithms that require carbon intensity forecasts under erroneous predictions, we have introduced random errors to carbon intensity data, denoted as $CI_{err}$, where $err$ is the mean of added error.


\noindent \textbf{Scaling Profiles:}
Carbon savings highly depend on the scalability of jobs~\cite{Hanafy:23:CarbonScaler}, where more scalable jobs can yield higher savings as they provide higher marginal throughput for each added resource. We adopt scaling profiles from ~\cite{Hanafy:23:CarbonScaler} and augment them with the special case of linearly scalable jobs \wa{verify when finalize the experiments}. However, since the online conversion algorithm requires a non-discrete scaling profile, we capture the scalability profiles by fitting the profiles to quadratic polynomial functions with 0 intercepts since assigning 0 servers should not yield any progress. Figure~\ref{fig:scalingprofiles} depicts the utilized scaling profiles their polynomial functions \wa{Plot the profiles}.


\noindent \textbf{Parameter settings:}
We construct various settings to benchmark our proposed algorithm. The settings includes evaluating the impact of minimum and maximum job length ($c_{\min}$ and $c_{\max}$), switching cost $\beta$, job length prediction error,  combination factors $\lambda$, carbon intensity prediction errors $CI_{err}$, rate constraints, and scaling profiles. In each setting, we uniformly sample a job length $\in$[\cmin, \cmax], and provide the algorithm with predicted length based on the expected error. 

\noindent \textbf{Baselines Algorithms:}
We evaluate our proposed algorithm, denoted as \aug, against state-of-the-art policies to include:
1) Online conversion with switching costs with knowledge of job length, denoted as \RORO \cite{Lechowicz:24}, 
2) One-Way Trading with job length prediction \OWT \cite{ElYaniv:01}, 
3) \threshold\cite{Wiesner:21} an online policy that switches between pausing and maximum rate based on a threshold, which we set at $\sqrt{UL}$, 
4) \agnostic, which runs at maximum rate when the job is submitted, and 
5) \carbonscaler \cite{Hanafy:23:CarbonScaler} utilizes the job and carbon intensity predictions to construct a carbon-aware schedule.
Finally, we highlight that all algorithms, except \RORO, will start the compulsory trade, i.e., run at the maximum rate when the remaining time is sufficient to fulfill the worst-case job length.


\noindent \textbf{Evaluation Metrics:}
The performance of the tested algorithms is evaluated in comparison to an offline optimal schedule computed using a numerical solver \cite{SciPy}, which allows us to report the empirical competitive ratio. \wa{We can move to earlier}% of several techniques in section \ref{sec:exp:numerical}. Then, we evaluate the performance of our algorithm in real-world settings (section \ref{sec:exp:real}) with respect to the carbon savings \% \wa{decide on metrics }compared to the \agnostic policy.



\begin{figure*}
    \centering
    \includegraphics[width=0.8\textwidth]{figures/sec1/cMax/cmax_labels.pdf}\\
    \begin{subfigure}[b]{0.245\textwidth}
        \centering
        \includegraphics[width=\textwidth, height=2.5cm]{figures/sec1/cMax/cmax_effect_1.png}
        \caption{\cmax= 1}
        \label{fig:effect_cMax_1}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.245\textwidth}
        \centering
        \includegraphics[width=\textwidth, height=2.5cm]{figures/sec1/cMax/cmax_effect_3.png}
        \caption{\cmax= 3}
        \label{fig:effect_cMax_3}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.245\textwidth}
        \centering
        \includegraphics[width=\textwidth, height=2.5cm]{figures/sec1/cMax/cmax_effect_6.png}
        \caption{\cmax = 6}
        \label{fig:effect_cMax_6}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.245\textwidth}
        \centering
        \includegraphics[width=\textwidth, height=2.5cm]{figures/sec1/cMax/cmax_effect.png}
        \caption{Effect of \cmax}
        \label{fig:effect_cMax_all}
    \end{subfigure}
    \caption{Cumulative distribution functions (CDFs) of empirical competitive ratios for selected algorithms under different \cmax values, where \cmin=1. d) Shows the effect of \cmax on average ALG/OPT. We assume $\beta=20$, job prediction error is $20\%$, $\lambda=0.5$, and the deadline of 24hrs.}
    \label{fig:effect_cMax}
\end{figure*}

\begin{figure*}
    \centering
    \includegraphics[width=0.8\textwidth]{figures/sec1/beta/beta_labels.pdf}\\
    \begin{subfigure}[b]{0.24\textwidth}
        \centering
        \includegraphics[width=\textwidth, height=2.5cm]{figures/sec1/beta/beta_effect_0.png}
        \caption{$\beta = 0$}
        \label{fig:effect_beta_0}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.24\textwidth}
        \centering
        \includegraphics[width=\textwidth, height=2.5cm]{figures/sec1/beta/beta_effect_20.png}
        \caption{$\beta = 20$}
        \label{fig:effect_beta_20}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.24\textwidth}
        \centering
        \includegraphics[width=\textwidth, height=2.5cm]{figures/sec1/beta/beta_effect_40.png}
        \caption{$\beta = 40$}
        \label{fig:effect_beta_40}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.24\textwidth}
        \centering
        \includegraphics[width=\textwidth, height=2.5cm]{figures/sec1/beta/beta_effect.png}
        \caption{Effect of $\beta$}
        \label{fig:effect_beta_all}
    \end{subfigure}
    \caption{Cumulative distribution functions (CDFs) of empirical competitive ratios for selected algorithms under different $\beta$ values. d) Shows the effect of $\beta$ on average ALG/OPT. We assume \cmax$=3$, job prediction error is $20$\%, $\lambda$=$0.5$, and deadline of 24hrs.}
    \label{fig:effect_beta}
\end{figure*}

\subsection{Numerical Experiments Results}\label{sec:exp:numerical}
\wa{state the profile}
In this section, we present a numerical evaluation of the proposed algorithm to \RORO, \OWT, \threshold, and \agnostic by showing their performance compared to an offline optimal algorithm\footnote{We leave out \carbonscaler as horizontal scaling requires discrete resource allocation.}. In this section, we do not enforce other constraints, such as rate constraints and discrete assignment, but will revisit them in section \ref{sec:exp:real}.

\subsubsection{Effect of maximum jobs length \cmax}
The relation between the maximum and minimum job length (\cmax/\cmin) dictates the distribution of jobs that the scheduler might face, where a higher ratio means a more diverse job length. For simplicity, we assume \cmin$=1$ and test against different values of \cmax. Figure \ref{fig:effect_cMax} shows the performance of various algorithms under different \cmax values, where lower ALG/OPT is better. We assume a fixed switching cost $\beta=20$, job prediction error of $20\%$, combination factor $\lambda=0.5$, and deadline of 24hrs.
Figure \ref{fig:effect_cMax_1} shows the special case where \cmax=\cmin, i.e., all jobs are the same length and known to \aug,  \RORO, \OWT. As expected, the results indicate that \aug and \RORO become identical while \OWT is a little behind as it does not consider switching costs. Nonetheless, these algorithms achieve higher performance than \threshold and \agnostic. 
Figure \ref{fig:effect_cMax_3} and \ref{fig:effect_cMax_6} other cases where the \cmax is 3 and 6, respectively. As shown, \aug performs the closest to \RORO in all settings and performs 3.3 and 8.6\% on average and 8.3 and 32.8\% in the worst case, worse than \RORO when \cmax is 3 and 6, respectively. \wa{Describe how \cmax affect the threshold function and how it ultimately affect the decisions made by \aug.}
Figure \ref{fig:effect_cMax_all} summarizes the average competitive ratio across different \cmax values. Interestingly, the results show that increasing the \cmax decreases the performance of all techniques but never changes their order.





\subsubsection{Effect of switching cost $\beta$}
Dynamic resource adjustment leads to wasted time and energy, known as switching costs. For example, the energy consumed by a server to switch on or off is its switching cost. Similarly, when applications employ suspend-resume scheduling, the switching cost is the incurred energy to checkpoint or restore the state before being able to resume processing. Although switching costs can vary dynamically according to the state or the current cost, for simplicity, we employ a fixed and symmetrical maximum switching cost $\beta$ that is paid when the algorithm scales from 0 to the maximum rate at any time slot. Figure \ref{fig:effect_beta} shows the performance of the algorithms against distinctive values of $\beta$.  We assume that \cmax$=3$, job prediction error is $20\%$, combination factor $\lambda=0.5$, and deadline of 24hrs.
We assigned $\beta$ as 10, 20, 30, and 40 gCO2eq, representing 3.6, 7.3, 10.9, and 14.6\% of California's average hourly carbon intensity (~273 gCO2eq/kWh). For completeness, we added the case of $\beta=0$ where resource scaling does not incur any overheads. As expected, \aug outperforms all other algorithms and closely matches the performance of \RORO. 
Figure \ref{fig:effect_beta_0} shows the case where switching is cost-free, where the performance of \aug, \OWT are almost identical. 
Figures \ref{fig:effect_beta_20} and \ref{fig:effect_beta_40} explore realistic cases with non-zero switching cost, where \aug outperforms \OWT on average in the worst case by 6.1 and 7.2\% when $\beta=20$ and by 13.8 and 38.8 when $\beta=40$. Finally, Figure \ref{fig:effect_beta_all} summarizes the average performance of all the algorithms, highlighting the effectiveness of our proposed approach.








\begin{figure*}
    \centering
    \begin{subfigure}[b]{0.24\textwidth}
        \centering
        \includegraphics[width=\textwidth, height=2.5cm]{figures/sec1/lambda_error/lambda_error_3_0.png}
        \caption{$\beta = 0$}
        \label{fig:lambda_error_3_0}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.2\textwidth}
        \centering
        \includegraphics[width=\textwidth, height=2.5cm]{figures/sec1/lambda_error/lambda_error_3_10.png}
        \caption{$\beta = 10$}
        \label{fig:lambda_error_3_10}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.2\textwidth}
        \centering
        \includegraphics[width=\textwidth, height=2.5cm]{figures/sec1/lambda_error/lambda_error_3_20.png}
        \caption{$\beta = 20$}
        \label{fig:lambda_error_3_20}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.24\textwidth}
        \centering
        \includegraphics[width=\textwidth, height=2.55cm]{figures/sec1/lambda_error/lambda_error_3_40.png}
        \caption{$\beta = 40$}
        \label{fig:lambda_error_3_40}
    \end{subfigure}
    \caption{ Lambda error \cmax=3}
    \label{fig:lambda_error_3}
\end{figure*}


\begin{figure*}
    \centering
    \begin{subfigure}[b]{0.24\textwidth}
        \centering
        \includegraphics[width=\textwidth, height=2.5cm]{figures/sec1/lambda_error/lambda_error_6_0.png}
        \caption{$\beta = 0$}
        \label{fig:lambda_error_6_0}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.2\textwidth}
        \centering
        \includegraphics[width=\textwidth, height=2.5cm]{figures/sec1/lambda_error/lambda_error_6_10.png}
        \caption{$\beta = 10$}
        \label{fig:lambda_error_6_10}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.2\textwidth}
        \centering
        \includegraphics[width=\textwidth, height=2.5cm]{figures/sec1/lambda_error/lambda_error_6_20.png}
        \caption{$\beta = 20$}
        \label{fig:lambda_error_6_20}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.24\textwidth}
        \centering
        \includegraphics[width=\textwidth, height=2.55cm]{figures/sec1/lambda_error/lambda_error_6_40.png}
        \caption{$\beta = 40$}
        \label{fig:lambda_error_6_40}
    \end{subfigure}
    \caption{ Lambda error \cmax=6}
    \label{fig:lambda_error_6}
\end{figure*}


\begin{figure*}
    \centering
    \includegraphics[width=0.45\textwidth]{figures/sec2/integer_error/cdf_integer_labels.pdf}\\
    \begin{subfigure}[b]{0.24\textwidth}
        \centering
        \includegraphics[width=\textwidth, height=2.5cm]{figures/sec2/integer_error/cdf_integer_0.png}
        \caption{$CI_{err}=0$}
        \label{fig:effect_int_carbon_err_0}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.24\textwidth}
        \centering
        \includegraphics[width=\textwidth, height=2.5cm]{figures/sec2/integer_error/cdf_integer_10.png}
        \caption{$CI_{err}=10\%$}
        \label{fig:effect_int_carbon_err_10}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.24\textwidth}
        \centering
        \includegraphics[width=\textwidth, height=2.5cm]{figures/sec2/integer_error/cdf_integer_40.png}
        \caption{$CI_{err}=40\%$}
        \label{fig:effect_int_carbon_err_40}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.24\textwidth}
        \centering
        \includegraphics[width=\textwidth, height=2.5cm]{figures/sec2/integer_error/cdf_integer_all.png}
    \caption{Effect of $CI_{err}$}
        \label{fig:effect_int_carbon_err_all}
    \end{subfigure}
    \caption{Cumulative distribution functions (CDFs) of empirical competitive ratios for selected algorithms under different $CI_{erro}$ values. d) Shows the effect of $CI_{err}$ on average ALG/OPT. We assume \cmax$=3$, $\beta=20$ job prediction error is $30\%$, $\lambda=0.5$, and deadline of 24hrs.}
    \label{fig:effect_int_carbon_err}
\end{figure*}

\subsection{Real-world Experimental Results}\label{sec:exp:real}



\subsubsection{Carbon Intensity error}
See figure \ref{fig:effect_int_carbon_err}

\begin{figure}
    \centering
     \begin{subfigure}[b]{0.236\textwidth}
        \centering
        \includegraphics[width=\textwidth, height=2.5cm]{figures/sec2/rates_30_10.png}
        \caption{$CI_{err}=10\%$}
    \label{fig:rate_10}
    \end{subfigure}
    \begin{subfigure}[b]{0.236\textwidth}
        \centering
        \includegraphics[width=\textwidth, height=2.5cm]{figures/sec2/rates_30_20.png}
        \caption{$CI_{err}=20\%$}
    \label{fig:rate_20}
    \end{subfigure}
    \caption{Rates}
    \label{fig:rates}
\end{figure}
\subsubsection{Rate}
See figure \ref{fig:rates}


\begin{figure}
    \centering
    \includegraphics[width=0.4\textwidth]{figures/sec2/profiles_AugmentINT_C.png}
    \caption{Profiles \wa{I think this graph shows that as scaling decreases we are less able to follow the optimal which is a negative message.}}
    \label{fig:profiles_augment}
\end{figure}

\subsection{Profiles}
See figure \ref{fig:profiles_augment}
